An Experiment on the Simulation of Deterministic Turing Machines by Large Language Models

Recent studies have shown that the use of chain-of-thought (CoT) under suitable assumptions enables large language models (LLMs) and transformers in general to achieve Turing completeness. In this paper, we put this claim to the test. We evaluate empirically the feasibility of using state-of-art LLMs with zero-shot CoT prompting to simulate arbitrary deterministic Turing machines. We tested four flagship models (DeepSeek V4 Pro, Gemini 2.5 Pro, GPT 5.4 and 5.2) over 116 randomly generated Turing machines with varying configurations. As expected, accuracy drops as the number of transitions of the simulated machine grows, but some models/modes of operation perform notably better than others, which corroborates the results of a related benchmark.

==> LLMUniversal.tex <==
\section{Introduction}

Large Language Models (LLMs) have recently been shown to exhibit computational capabilities that go far beyond natural language processing. In particular, several theoretical and empirical studies suggest that Transformer architectures can simulate Turing Machines and, under suitable assumptions, achieve Turing completeness. These results have motivated a growing body of research investigating the algorithmic capabilities and limitations of modern language models.

Despite these advances, an important distinction must be made between the computational power of the underlying Transformer architecture and the practical behavior of deployed LLMs. While a Transformer may be theoretically capable of simulating arbitrary computations, the actual execution performed by a pretrained language model is inherently stochastic and therefore subject to errors. This raises a fundamental question: can prompts themselves be regarded as executable specifications of computational systems?

In this work, we investigate this question through the construction of a prompt-based Universal Turing Machine (UTM). Rather than modifying the model architecture or retraining the network, we encode the operational semantics of a Universal Turing Machine directly as a prompt and use the LLM as the execution engine. Given a deterministic Turing Machine $T$ and an input word $w$, the prompt instructs the model to simulate the successive configurations of $T$.

Since LLM outputs are probabilistic, a direct execution may deviate from the intended transition function. To address this issue, we developed an independent verification program that checks every generated configuration against the formal specification of the simulated machine. Whenever an incorrect transition is detected, the execution is interrupted and classified as a failure. This allows us to evaluate the prompt not merely as a text-generation artifact but as an executable computational specification whose correctness can be objectively measured.

The use of prompts as computational descriptions is particularly interesting because prompts operate at a significantly higher level of abstraction than Transformer weights. Consequently, they may offer advantages in transparency, portability, and ease of implementation. On the other hand, the additional abstraction layer may introduce new sources of computational error, making deterministic execution more challenging.

The objective of this paper is therefore not to establish the computational universality of LLMs, which has already been extensively discussed in the literature, but rather to evaluate the practical feasibility of prompt-based computation. We experimentally investigate the reliability of prompt-driven simulations of deterministic Turing Machines and compare the observed behavior with previous reports on Transformer-based Turing Machine implementations. We also relate our findings to classical universal computational formalisms, particularly Universal Post Systems, whose rule-based operational character resembles the symbolic execution induced by prompts, as reported in \cite{chineses}.

Our results provide quantitative evidence regarding the degree to which deterministic symbolic computation can be achieved through prompting alone. More broadly, they contribute to understanding the relationship between formal models of computation and modern generative AI systems, clarifying the extent to which prompts can serve as executable computational artifacts rather than merely natural-language instructions.

